Vis2Mesh: Efficient Mesh Reconstruction from Unstructured Point Clouds of Large Scenes with Learned Virtual View Visibility

We present a novel framework for mesh reconstruction from unstructured point clouds by taking advantage of the learned visibility of the 3D points in the virtual views and traditional graph-cut based mesh generation. Specifically, we first propose a three-step network that explicitly employs depth completion for visibility prediction. Then the visibility information of multiple views is aggregated to generate a 3D mesh model by solving an optimization problem considering visibility in which a novel adaptive visibility weighting in surface determination is also introduced to suppress line of sight with a large incident angle. Compared to other learning-based approaches, our pipeline only exercises the learning on a 2D binary classification task, \ie, points visible or not in a view, which is much more generalizable and practically more efficient and capable to deal with a large number of points. Experiments demonstrate that our method with favorable transferability and robustness, and achieve competing performances \wrt state-of-the-art learning-based approaches on small complex objects and outperforms on large indoor and outdoor scenes. Code is available at https://github.com/GDAOSU/vis2mesh.

==> exp_imgs/exp_figures.tex <==
\usepackage{graphicx}
\usepackage[caption=false]{subfig}
\graphicspath{ {exp_imgs/}}

\newcommand{\mkfigReconDSLRViewOne}[2]{
\begin{figure} 
    \def\subimgwidth{0.45\linewidth}
    \edef\trimopts{trim=200 100 300 50,clip,width = \subimgwidth}
    
    \centering
    \setlength{\tabcolsep}{2pt}
    \def\arraystretch{0}
    \begin{tabular}{cc}
    \subfloat[P2M]{%
        \expandafter\includegraphics\expandafter[\trimopts]{object_dslr/point2mesh_view_1.png}}&
    \subfloat[P2S]{%
        \expandafter\includegraphics\expandafter[\trimopts]{object_dslr/p2s_view_1.png}}\\
    \subfloat[MIER]{%
        \expandafter\includegraphics\expandafter[\trimopts]{object_dslr/mier_view_1.png}}&
    \subfloat[CONet]{%
        \expandafter\includegraphics\expandafter[\trimopts]{object_dslr/convonet_view_1.png}}\\
    \subfloat[Poisson]{%
        \expandafter\includegraphics\expandafter[\trimopts]{object_dslr/poisson_view_1.png}}&
    \subfloat[Ours]{%
        \expandafter\includegraphics\expandafter[\trimopts]{object_dslr/ours_angle_view_1.png}}
    \end{tabular}
  
  \caption{#1}
  \label{#2} 
\end{figure}
}

\newcommand{\mkfigReconDSLRViewTwo}[2]{\begin{figure} 
    \def\subimgwidth{0.45\linewidth}
    \edef\trimopts{trim=200 10 300 50,clip,width = \subimgwidth}
    
    \centering
    \setlength{\tabcolsep}{2pt}
    \def\arraystretch{0}
    \begin{tabular}{cc}
    \subfloat[P2M]{%
        \expandafter\includegraphics\expandafter[\trimopts]{object_dslr/point2mesh_view_2.png}}&
    \subfloat[P2S]{%
        \expandafter\includegraphics\expandafter[\trimopts]{object_dslr/p2s_view_2.png}}\\
    \subfloat[MIER]{%
        \expandafter\includegraphics\expandafter[\trimopts]{object_dslr/mier_view_2.png}}&
    \subfloat[CONet]{%
       \expandafter\includegraphics\expandafter[\trimopts]{object_dslr/convonet_view_2.png}}\\
    \subfloat[Poisson]{%
        \expandafter\includegraphics\expandafter[\trimopts]{object_dslr/poisson_view_2.png}}&
    \subfloat[Ours]{%
        \expandafter\includegraphics\expandafter[\trimopts]{object_dslr/ours_angle_view_2.png}}
    \end{tabular}

  \caption{#1}
  \label{#2} 
\end{figure}}

\newcommand{\mkfigReconRoomZeroViewOne}[2]{\begin{figure} 
    \def\subimgwidth{0.45\linewidth}
    \edef\trimopts{trim=350 0 230 165,clip,width = \subimgwidth}
    
    \centering
    \setlength{\tabcolsep}{2pt}
    \def\arraystretch{0}
    \begin{tabular}{cc}
    \subfloat[Input Points]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_0_raw/pointcloud_ramp_view_1.png}}&
    \subfloat[P2S]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_0_raw/p2s_view_1.png}}\\
    \subfloat[MIER]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_0_raw/mier_view_1.png}}&
    \subfloat[CONet]{%
       \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_0_raw/convonet_view_1.png}}\\
    \subfloat[Poisson]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_0_raw/poisson_view_1.png}}&
    \subfloat[Ours]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_0_raw/ours_view_1.png}}
    \end{tabular}
    
  \caption{#1}
  \label{#2} 
\end{figure}}

\newcommand{\mkfigReconRoomOneViewOne}[2]{
\begin{figure} 
    \def\subimgwidth{0.45\linewidth}
    \edef\trimopts{trim=300 30 230 50,clip,width = \subimgwidth}
    
    \centering
    \setlength{\tabcolsep}{2pt}
    \def\arraystretch{0}
    \begin{tabular}{cc}
    \subfloat[Input Points]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_1_raw/pointcloud_ramp_view_1.png}}&
    \subfloat[P2S]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_1_raw/p2s_view_1.png}}\\
    \subfloat[MIER]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_1_raw/mier_view_1.png}}&
    \subfloat[CONet]{%
       \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_1_raw/convonet_view_1.png}}\\
    \subfloat[Poisson]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_1_raw/poisson_view_1.png}}&
    \subfloat[Ours]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_1_raw/ours_view_1.png}}
    \end{tabular}
    
  \caption{#1}
  \label{#2} 
\end{figure}}

\newcommand{\mkfigReconRoomOneViewTwo}[2]{
\begin{figure} 
\def\subimgwidth{0.45\linewidth}
    \edef\trimopts{trim=300 30 230 50,clip,width = \subimgwidth}
    
    \centering
    \setlength{\tabcolsep}{2pt}
    \def\arraystretch{0}
    \begin{tabular}{cc}
    \subfloat[Input Points]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_1_raw/pointcloud_ramp_view_2.png}}&
    \subfloat[P2S]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_1_raw/p2s_view_2.png}}\\
    \subfloat[MIER]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_1_raw/mier_view_2.png}}&
    \subfloat[CONet]{%
       \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_1_raw/convonet_view_2.png}}\\
    \subfloat[Poisson]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_1_raw/poisson_view_2.png}}&
    \subfloat[Ours]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_1_raw/ours_view_2.png}}
    \end{tabular}

  \caption{#1}
  \label{#2} 
\end{figure}}

\newcommand{\mkfigReconSmallObjects}[2]{
\begin{figure}
    \def\subimgwidth{0.14\linewidth}
    \edef\bullopts{trim=310 30 340 75,clip,width = \subimgwidth}
    \edef\triopts{trim=290 60 260 120,clip,width = \subimgwidth}
    \edef\grfopts{trim=370 0 510 15,clip,width = \subimgwidth}
    \edef\grfheadopts{trim=320 80 350 20,clip,width = \subimgwidth}
    \edef\tikiopts{trim=370 0 495 20,clip,width = \subimgwidth}

    \centering
    \setlength{\tabcolsep}{0pt}
    \def\arraystretch{0}
    \begin{tabular}{ccccccc} 
    \subfloat[Input]{%
    \begin{tabular}{c}
         \expandafter\includegraphics\expandafter[\bullopts]{object_bull/pointcloud_ramp_view_1.png} \\
         \expandafter\includegraphics\expandafter[\triopts]{object_triceratops_raw/pointcloud_ramp_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfopts]{object_giraffe/pointcloud_ramp_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfheadopts]{object_giraffe/pointcloud_ramp_view_2.png} \\
         \expandafter\includegraphics\expandafter[\tikiopts]{object_tiki/pointcloud_ramp_view_1.png}
    \end{tabular}} &
    \subfloat[P2M]{%
    \begin{tabular}{c}
         \expandafter\includegraphics\expandafter[\bullopts]{object_bull/point2mesh_view_1.png} \\ 
         \expandafter\includegraphics\expandafter[\triopts]{object_triceratops_raw/point2mesh_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfopts]{object_giraffe/point2mesh_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfheadopts]{object_giraffe/point2mesh_view_2.png} \\
         \expandafter\includegraphics\expandafter[\tikiopts]{object_tiki/point2mesh_view_1.png}
    \end{tabular}} &
    \subfloat[P2S]{%
    \begin{tabular}{c}
         \expandafter\includegraphics\expandafter[\bullopts]{object_bull/p2s_view_1.png} \\ 
         \expandafter\includegraphics\expandafter[\triopts]{object_triceratops_raw/p2s_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfopts]{object_giraffe/p2s_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfheadopts]{object_giraffe/p2s_view_2.png} \\
         \expandafter\includegraphics\expandafter[\tikiopts]{object_tiki/p2s_view_1.png}
    \end{tabular}} &
    \subfloat[MIER]{%
    \begin{tabular}{c}
         \expandafter\includegraphics\expandafter[\bullopts]{object_bull/mier_view_1.png} \\ 
         \expandafter\includegraphics\expandafter[\triopts]{object_triceratops_raw/mier_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfopts]{object_giraffe/mier_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfheadopts]{object_giraffe/mier_view_2.png} \\
         \expandafter\includegraphics\expandafter[\tikiopts]{object_tiki/mier_view_1.png}
    \end{tabular}} &
    \subfloat[CONet]{%
    \begin{tabular}{c}
        \expandafter\includegraphics\expandafter[\bullopts]{object_bull/convonet_view_1.png} \\
        \expandafter\includegraphics\expandafter[\triopts]{object_triceratops_raw/convonet_view_1.png} \\ 
        \expandafter\includegraphics\expandafter[\grfopts]{object_giraffe/convonet_view_1.png} \\
        \expandafter\includegraphics\expandafter[\grfheadopts]{object_giraffe/convonet_view_2.png} \\
        \expandafter\includegraphics\expandafter[\tikiopts]{object_tiki/convonet_view_1.png}
    \end{tabular}} &
    \subfloat[Poisson]{%
    \begin{tabular}{c}
         \expandafter\includegraphics\expandafter[\bullopts]{object_bull/poisson_view_1.png} \\
         \expandafter\includegraphics\expandafter[\triopts]{object_triceratops_raw/poisson_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfopts]{object_giraffe/poisson_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfheadopts]{object_giraffe/poisson_view_2.png} \\
         \expandafter\includegraphics\expandafter[\tikiopts]{object_tiki/poisson_view_1.png}
    \end{tabular}} &
    \subfloat[Ours]{%
    \begin{tabular}{c}
        \expandafter\includegraphics\expandafter[\bullopts]{object_bull/ours_view_1.png} \\
        \expandafter\includegraphics\expandafter[\triopts]{object_triceratops_raw/ours_view_1.png} \\
        \expandafter\includegraphics\expandafter[\grfopts]{object_giraffe/ours_view_1.png} \\
        \expandafter\includegraphics\expandafter[\grfheadopts]{object_giraffe/ours_view_2.png} \\
        \expandafter\includegraphics\expandafter[\tikiopts]{object_tiki/ours_view_1.png} 
    \end{tabular}}
    \end{tabular}
%%%%%%%%%%%%
\caption{#1}
\label{#2}
\end{figure}}

\newcommand{\mkfigReconSingleFloor}[2]{
\begin{figure}
    \def\subimgwidth{0.48\linewidth}
    \edef\trimopts{trim=20 48 10 63,clip,width = \subimgwidth}

    \centering
    \setlength{\tabcolsep}{2pt}
    \def\arraystretch{0}
    \begin{tabular}{cc}
    \subfloat[Input Points]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_matterport_singlefloor/pointcloud_ramp_view_1.png}} &
    \subfloat[CONet]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_matterport_singlefloor/convonet_view_1.png}} \\
    \subfloat[Poisson]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_matterport_singlefloor/poisson_view_1.png}} &
    \subfloat[Ours]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_matterport_singlefloor/ours_view_1.png}}
    \end{tabular}
    
    \caption{#1}
    \label{#2}
\end{figure}}

\newcommand{\mkfigReconMultiFloor}[2]{
\begin{figure}
    \def\subimgwidth{0.48\linewidth}
    \edef\trimopts{trim=100 10 200 50,clip,width = \subimgwidth}

    \centering
    \setlength{\tabcolsep}{2pt}
    \def\arraystretch{0}
    \begin{tabular}{cc}
    \subfloat[Input Points]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_matterport_multifloor/pointcloud_ramp_view_1.png}} &
    \subfloat[CONet]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_matterport_multifloor/convonet_view_1.png}} \\
    \subfloat[Poisson]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_matterport_multifloor/poisson_view_1.png}} &
    \subfloat[Ours]{%
        \expandafter\includegraphics\expandafter[\trimopts]{indoor_matterport_multifloor/ours_view_1.png}}
    \end{tabular}

    \caption{#1}
    \label{#2}
\end{figure}}

\newcommand{\mkfigReconAirbornelidar}[2]{
\begin{figure}
    \def\subimgwidth{0.3\linewidth}
    \edef\trtCopts{trim=190 60 380 50,clip,width = \subimgwidth}
    \edef\trtDopts{trim=200 80 300 70,clip,width = \subimgwidth}
    \edef\clbBopts{trim=0 0 0 20,clip,width = \subimgwidth}
    
    \centering
    \setlength{\tabcolsep}{1pt}
    \def\arraystretch{1}
    \begin{tabular}{ccc} 
    \subfloat[Input Points]{%
    \begin{tabular}{c}
         \expandafter\includegraphics\expandafter[\trtCopts]{largescale_toronto/pointcloud_ramp_view_3.png} \\
         \expandafter\includegraphics\expandafter[\trtDopts]{largescale_toronto/pointcloud_ramp_view_4.png} \\
         \expandafter\includegraphics\expandafter[\clbBopts]{largescale_columbus/pointcloud_ramp_view_2.png}
    \end{tabular}} &
    \subfloat[CONet]{%
    \begin{tabular}{c}
         \expandafter\includegraphics\expandafter[\trtCopts]{largescale_toronto/convonet_view_3.png} \\
         \expandafter\includegraphics\expandafter[\trtDopts]{largescale_toronto/convonet_view_4.png} \\
         \expandafter\includegraphics\expandafter[\clbBopts]{largescale_columbus/convonet_view_2.png}
    \end{tabular}} &
    \subfloat[Ours]{%
    \begin{tabular}{c}
         \expandafter\includegraphics\expandafter[\trtCopts]{largescale_toronto/ours_view_3.png} \\
         \expandafter\includegraphics\expandafter[\trtDopts]{largescale_toronto/ours_view_4.png} \\
         \expandafter\includegraphics\expandafter[\clbBopts]{largescale_columbus/ours_view_2.png}
    \end{tabular}}
    \end{tabular}
    
    \caption{#1}
    \label{#2}
\end{figure}}

\newcommand{\mkfigReconHKUSTViewOne}[2]{
\begin{figure}
    \def\subimgwidth{0.48\linewidth}
    \edef\trimopts{trim=0 0 200 0,clip,width = \subimgwidth}
    
    \centering
    \setlength{\tabcolsep}{2pt}
    \def\arraystretch{0}
    \begin{tabular}{cc}
    \subfloat[Input Points]{%
        \expandafter\includegraphics\expandafter[\trimopts]{largescale_hkust_building1/pointcloud_view_1.png}} &
    \subfloat[CONet]{%
       \expandafter\includegraphics\expandafter[\trimopts]{largescale_hkust_building1/convonet_view_1.png}} \\
    \subfloat[Poisson]{%
        \expandafter\includegraphics\expandafter[\trimopts]{largescale_hkust_building1/poisson_view_1.png}} &
    \subfloat[Ours]{%
        \expandafter\includegraphics\expandafter[\trimopts]{largescale_hkust_building1/ours_view_1.png}}
    \end{tabular}
    
    \caption{#1}
    \label{#2}
\end{figure}}

\newcommand{\mkfigReconHKUSTViewTwo}[2]{
\begin{figure}
    \def\subimgwidth{0.48\linewidth}
    \edef\trimopts{trim=0 0 200 0,clip,width = \subimgwidth}
    
    \centering
    \setlength{\tabcolsep}{2pt}
    \def\arraystretch{0}
    \begin{tabular}{cc}
    \subfloat[Input Points]{%
        \expandafter\includegraphics\expandafter[\trimopts]{largescale_hkust_building1/pointcloud_view_2.png}} &
    \subfloat[CONet]{%
       \expandafter\includegraphics\expandafter[\trimopts]{largescale_hkust_building1/convonet_view_2.png}} \\
    \subfloat[Poisson]{%
        \expandafter\includegraphics\expandafter[\trimopts]{largescale_hkust_building1/poisson_view_2.png}} &
    \subfloat[Ours]{%
        \expandafter\includegraphics\expandafter[\trimopts]{largescale_hkust_building1/ours_view_2.png}}
    \end{tabular}

    \caption{#1}
    \label{#2}
\end{figure}}


\newcommand{\mkfigAngleDecayRoomOne}[2]{
\begin{figure}
    \def\subimgwidth{0.4\linewidth}
    \edef\sinkopts{trim=350 50 400 0,clip,width = \subimgwidth}
    \edef\lampopts{trim=400 50 400 0,clip,width = \subimgwidth}
    
    \centering
    \setlength{\tabcolsep}{1pt}
    \def\arraystretch{1}
    \begin{tabular}{cc}
    \subfloat[Without angle decay]{%
    \begin{tabular}{c}
    \expandafter\includegraphics\expandafter[\sinkopts]{indoor_room_1_raw/ours_view_3.png}\\
    \expandafter\includegraphics\expandafter[\lampopts]{indoor_room_1_raw/ours_view_4.png}
    \end{tabular}}&
    \subfloat[With angle decay]{%
    \begin{tabular}{c}
    \expandafter\includegraphics\expandafter[\sinkopts]{indoor_room_1_raw/ours_angle_view_3.png}\\
    \expandafter\includegraphics\expandafter[\lampopts]{indoor_room_1_raw/ours_angle_view_4.png}
    \end{tabular}}
    \end{tabular}

    \caption{#1}
    \label{#2}
\end{figure}}


\newcommand{\mkfigTypeOfNoises}[2]{
\begin{figure}
    \def\subimgwidth{0.3\linewidth}
    \edef\trimopts{trim=290 60 260 120,clip,width = \subimgwidth}
    
    \centering
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{ccc}
    \subfloat[Raw]{%
    \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_0_raw/pointcloud_ramp_view_1.png}} &
    \subfloat[Outlier Noise]{%
    \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_0_outlier/pointcloud_ramp_view_1.png}} &
    \subfloat[Gaussian Noise]{%
    \expandafter\includegraphics\expandafter[\trimopts]{indoor_room_0_noise/pointcloud_ramp_view_1.png}}
    \end{tabular}
    \caption{#1}
    \label{#2}
\end{figure}}

\newcommand{\mkfigNoiseEvalIndoor}[2]{
\begin{figure}
    \def\subimgwidth{0.3\linewidth}
    \edef\trimopt{trim=350 0 230 165,clip,clip,width = \subimgwidth}
    
    \centering
    \setlength\tabcolsep{1pt}
    \def\arraystretch{1}
    \begin{tabular}{cccc}
        & Noiseless & Outlier Noise & Gaussian Noise \\
        \rotatebox[origin=c]{90}{Input} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_raw/pointcloud_ramp_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_outlier/pointcloud_ramp_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_noise/pointcloud_ramp_view_1.png}} \\
        \rotatebox[origin=c]{90}{P2S} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_raw/p2s_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_outlier/p2s_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_noise/p2s_view_1.png}} \\
        \rotatebox[origin=c]{90}{MIER} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_raw/mier_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_outlier/mier_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_noise/mier_view_1.png}} \\
        \rotatebox[origin=c]{90}{CONet} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_raw/convonet_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_outlier/convonet_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_noise/convonet_view_1.png}} \\
        \rotatebox[origin=c]{90}{Poisson} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_raw/poisson_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_outlier/poisson_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_noise/poisson_view_1.png}} \\
        \rotatebox[origin=c]{90}{Ours} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_raw/ours_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_outlier/ours_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_noise/ours_view_1.png}}
        
    \end{tabular}
    \caption{#1}
    \label{#2}
\end{figure}}

\newcommand{\mkfigNoiseEvalSmallObject}[2]{
\begin{figure}
    \def\subimgwidth{0.3\linewidth}
    \edef\trimopt{trim=290 60 260 120,clip,clip,width = \subimgwidth}
    
    \centering
    \setlength\tabcolsep{1pt}
    \def\arraystretch{1}
    \begin{tabular}{cccc}
        & Noiseless & Outlier Noise & Gaussian Noise \\
        \rotatebox[origin=c]{90}{Input} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_raw/pointcloud_ramp_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_outlier/pointcloud_ramp_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_noise/pointcloud_ramp_view_1.png}} \\
        \rotatebox[origin=c]{90}{P2M} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_raw/point2mesh_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_outlier/point2mesh_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_noise/point2mesh_view_1.png}} \\
        \rotatebox[origin=c]{90}{P2S} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_raw/p2s_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_outlier/p2s_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_noise/p2s_view_1.png}} \\
        \rotatebox[origin=c]{90}{MIER} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_raw/mier_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_outlier/mier_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_noise/mier_view_1.png}} \\
        \rotatebox[origin=c]{90}{CONet} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_raw/convonet_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_outlier/convonet_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_noise/convonet_view_1.png}} \\
        \rotatebox[origin=c]{90}{Poisson} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_raw/poisson_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_outlier/poisson_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_noise/poisson_view_1.png}} \\
        \rotatebox[origin=c]{90}{Ours} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_raw/ours_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_outlier/ours_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{object_triceratops_noise/ours_view_1.png}} 
    \end{tabular}
    \caption{#1}
    \label{#2}
\end{figure}}

\newcommand{\mkfigViewEvalLandscape}[2]{
\begin{figure*}
    \def\subimgwidth{0.19\linewidth}
    \edef\trimopta{trim=270 0 300 0,clip,width = \subimgwidth}
    \edef\trimoptb{trim=120 50 140 145,clip,width = \subimgwidth}
    \edef\trimoptc{trim=60 100 620 90,clip,width = \subimgwidth}
    
    \centering
    \setlength\tabcolsep{1pt}
    \def\arraystretch{1}
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \expandafter\includegraphics\expandafter[\trimopta]{room_0_viewanalysis/orangecloud_c0_v1.png} &
        \expandafter\includegraphics\expandafter[\trimopta]{room_0_viewanalysis/orangecloud_c1_v1.png} &
        \expandafter\includegraphics\expandafter[\trimopta]{room_0_viewanalysis/orangecloud_c2_v1.png} &
        \expandafter\includegraphics\expandafter[\trimopta]{room_0_viewanalysis/orangecloud_c3_v1.png} &
        \expandafter\includegraphics\expandafter[\trimopta]{room_0_viewanalysis/orangecloud_c4_v1.png} \\\hline
        \expandafter\includegraphics\expandafter[\trimoptb]{room_0_viewanalysis/our0_v3.png} &
        \expandafter\includegraphics\expandafter[\trimoptb]{room_0_viewanalysis/our1_v3.png} &
        \expandafter\includegraphics\expandafter[\trimoptb]{room_0_viewanalysis/our2_v3.png} &
        \expandafter\includegraphics\expandafter[\trimoptb]{room_0_viewanalysis/our3_v3.png} &
        \expandafter\includegraphics\expandafter[\trimoptb]{room_0_viewanalysis/our4_v3.png} \\\hline
        \expandafter\includegraphics\expandafter[\trimoptc]{room_0_viewanalysis/our_c0_v2.png} &
        \expandafter\includegraphics\expandafter[\trimoptc]{room_0_viewanalysis/our_c1_v2.png} &
        \expandafter\includegraphics\expandafter[\trimoptc]{room_0_viewanalysis/our_c2_v2.png} &
        \expandafter\includegraphics\expandafter[\trimoptc]{room_0_viewanalysis/our_c3_v2.png} &
        \expandafter\includegraphics\expandafter[\trimoptc]{room_0_viewanalysis/our_c4_v2.png}
        \\\hline
        1 cam & 8 cams &
        14 cams & 22 cams &
        38 cams \\\hline
    \end{tabular}
    \caption{#1}
    \label{#2}
\end{figure*}}

\newcommand{\mkfigViewEvalPortrait}[2]{
\begin{figure*}
    \def\subimgheight{1.1 in}
    \edef\trimopta{trim=270 0 300 0,clip,height = \subimgheight}
    \edef\trimoptb{trim=120 40 140 145,clip,height = \subimgheight}
    \edef\trimoptc{trim=60 100 620 90,clip,height = \subimgheight}
    
    \centering
    \setlength\tabcolsep{1pt}
    \def\arraystretch{1}
    \begin{tabular}{|c|c|c|c|}
    \hline
    \rotatebox[origin=c]{90}{1 Cam} &
    \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopta]{room_0_viewanalysis/orangecloud_c0_v1.png}} &
    \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimoptb]{room_0_viewanalysis/our0_v3.png}} &
    \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimoptc]{room_0_viewanalysis/our_c0_v2.png}} \\\hline
    \rotatebox[origin=c]{90}{8 Cams} &
    \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopta]{room_0_viewanalysis/orangecloud_c1_v1.png}} &
    \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimoptb]{room_0_viewanalysis/our1_v3.png}} &
    \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimoptc]{room_0_viewanalysis/our_c1_v2.png}} \\\hline
    \rotatebox[origin=c]{90}{14 Cams} &
    \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopta]{room_0_viewanalysis/orangecloud_c2_v1.png}} &
    \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimoptb]{room_0_viewanalysis/our2_v3.png}} &
    \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimoptc]{room_0_viewanalysis/our_c2_v2.png}} \\\hline
    \rotatebox[origin=c]{90}{22 Cams} &
    \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopta]{room_0_viewanalysis/orangecloud_c3_v1.png}} &
    \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimoptb]{room_0_viewanalysis/our3_v3.png}} &
    \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimoptc]{room_0_viewanalysis/our_c3_v2.png}} \\\hline
    \rotatebox[origin=c]{90}{38 Cams} &
    \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopta]{room_0_viewanalysis/orangecloud_c4_v1.png}} &
    \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimoptb]{room_0_viewanalysis/our4_v3.png}} &
    \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimoptc]{room_0_viewanalysis/our_c4_v2.png}} \\\hline
    \end{tabular}
    
    \caption{#1}
    \label{#2}
\end{figure*}}


\newcommand{\mkfigReconEvalVisEstimatorsSmallObjects}[2]{
\begin{figure}
    \def\subimgwidth{0.25\linewidth}
    \edef\bullopts{trim=310 30 340 75,clip,width = \subimgwidth}
    \edef\triopts{trim=290 60 260 120,clip,width = \subimgwidth}
    \edef\grfopts{trim=370 0 510 15,clip,width = \subimgwidth}
    \edef\grfheadopts{trim=320 80 350 20,clip,width = \subimgwidth}
    \edef\tikiopts{trim=370 0 495 20,clip,width = \subimgwidth}

    \centering
    \setlength{\tabcolsep}{0pt}
    \def\arraystretch{0}
    \begin{tabular}{cccc} 
    \subfloat[Input]{%
    \begin{tabular}{c}
         \expandafter\includegraphics\expandafter[\bullopts]{object_bull/pointcloud_ramp_view_1.png} \\
         \expandafter\includegraphics\expandafter[\triopts]{object_triceratops_raw/pointcloud_ramp_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfopts]{object_giraffe/pointcloud_ramp_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfheadopts]{object_giraffe/pointcloud_ramp_view_2.png} \\
         \expandafter\includegraphics\expandafter[\tikiopts]{object_tiki/pointcloud_ramp_view_1.png}
    \end{tabular}} &
    \subfloat[UNet]{%
    \begin{tabular}{c}
         \expandafter\includegraphics\expandafter[\bullopts]{object_bull/unet_view_1.png} \\ 
         \expandafter\includegraphics\expandafter[\triopts]{object_triceratops_raw/unet_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfopts]{object_giraffe/unet_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfheadopts]{object_giraffe/unet_view_2.png} \\
         \expandafter\includegraphics\expandafter[\tikiopts]{object_tiki/unet_view_1.png}
    \end{tabular}} &
    \subfloat[HPR]{%
    \begin{tabular}{c}
         \expandafter\includegraphics\expandafter[\bullopts]{object_bull/hpr_view_1.png} \\ 
         \expandafter\includegraphics\expandafter[\triopts]{object_triceratops_raw/hpr_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfopts]{object_giraffe/hpr_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfheadopts]{object_giraffe/hpr_view_2.png} \\
         \expandafter\includegraphics\expandafter[\tikiopts]{object_tiki/hpr_view_1.png}
    \end{tabular}} &
    \subfloat[Ours]{%
    \begin{tabular}{c}
        \expandafter\includegraphics\expandafter[\bullopts]{object_bull/ours_view_1.png} \\
        \expandafter\includegraphics\expandafter[\triopts]{object_triceratops_raw/ours_view_1.png} \\
        \expandafter\includegraphics\expandafter[\grfopts]{object_giraffe/ours_view_1.png} \\
        \expandafter\includegraphics\expandafter[\grfheadopts]{object_giraffe/ours_view_2.png} \\
        \expandafter\includegraphics\expandafter[\tikiopts]{object_tiki/ours_view_1.png} 
    \end{tabular}}
    \end{tabular}
    
    \caption{#1}
    \label{#2}
\end{figure}}


\newcommand{\mkfigNoiseEvalVisEstimatorsIndoor}[2]{
\begin{figure}
    \def\subimgwidth{0.3\linewidth}
    \edef\trimopt{trim=350 0 230 165,clip,clip,width = \subimgwidth}
    
    \centering
    \setlength\tabcolsep{1pt}
    \def\arraystretch{1}
    \begin{tabular}{cccc}
        & Noiseless & Outlier Noise & Gaussian Noise \\
        \rotatebox[origin=c]{90}{Input} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_raw/pointcloud_ramp_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_outlier/pointcloud_ramp_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_noise/pointcloud_ramp_view_1.png}} \\
        \rotatebox[origin=c]{90}{UNet} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_raw/unet_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_outlier/unet_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_noise/unet_view_1.png}} \\
        \rotatebox[origin=c]{90}{HPR} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_raw/hpr_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_outlier/hpr_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_noise/hpr_view_1.png}} \\
        \rotatebox[origin=c]{90}{Ours} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_raw/ours_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_outlier/ours_view_1.png}} &
        \raisebox{-0.5\height}{\expandafter\includegraphics\expandafter[\trimopt]{indoor_room_0_noise/ours_view_1.png}}
        
    \end{tabular}
    \caption{#1}
    \label{#2}
\end{figure}}

\newcommand{\mkfigReconEvalVisEstimatorsSmallObjectsWithTrivial}[2]{
\begin{figure}
    \def\subimgwidth{0.2\linewidth}
    \edef\bullopts{trim=310 30 340 75,clip,width = \subimgwidth}
    \edef\triopts{trim=290 60 260 120,clip,width = \subimgwidth}
    \edef\grfopts{trim=370 0 510 15,clip,width = \subimgwidth}
    \edef\grfheadopts{trim=320 80 350 20,clip,width = \subimgwidth}
    \edef\tikiopts{trim=370 0 495 20,clip,width = \subimgwidth}
    \edef\roomZeroViewOneopts{trim=350 0 230 165,clip,width = \subimgwidth}
    \edef\roomOneViewTwoopts{trim=300 30 230 50,clip,width = \subimgwidth}
    \edef\DSLRViewOneopts{trim=200 100 300 50,clip,width = \subimgwidth}
    \centering
    \setlength{\tabcolsep}{0pt}
    \def\arraystretch{0}
    \begin{tabular}{ccccc} 
    \subfloat[Input]{%
    \begin{tabular}{c}
         \expandafter\includegraphics\expandafter[\bullopts]{object_bull/pointcloud_ramp_view_1.png} \\
         \expandafter\includegraphics\expandafter[\triopts]{object_triceratops_raw/pointcloud_ramp_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfopts]{object_giraffe/pointcloud_ramp_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfheadopts]{object_giraffe/pointcloud_ramp_view_2.png} \\
         \expandafter\includegraphics\expandafter[\tikiopts]{object_tiki/pointcloud_ramp_view_1.png} \\
         \expandafter\includegraphics\expandafter[\DSLRViewOneopts]{object_dslr/pointcloud_view_1.png} \\
         \expandafter\includegraphics\expandafter[\roomZeroViewOneopts]{indoor_room_0_raw/pointcloud_ramp_view_1.png} \\
         \expandafter\includegraphics\expandafter[\roomOneViewTwoopts]{indoor_room_1_raw/pointcloud_ramp_view_2.png}
    \end{tabular}} &
    \subfloat[Trivial]{%
    \begin{tabular}{c}
         \expandafter\includegraphics\expandafter[\bullopts]{object_bull/triv_view_1.png} \\ 
         \expandafter\includegraphics\expandafter[\triopts]{object_triceratops_raw/triv_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfopts]{object_giraffe/triv_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfheadopts]{object_giraffe/triv_view_2.png} \\
         \expandafter\includegraphics\expandafter[\tikiopts]{object_tiki/triv_view_1.png} \\
         \expandafter\includegraphics\expandafter[\DSLRViewOneopts]{object_dslr/triv_view_1.png} \\
         \expandafter\includegraphics\expandafter[\roomZeroViewOneopts]{indoor_room_0_raw/triv_view_1.png} \\
         \expandafter\includegraphics\expandafter[\roomOneViewTwoopts]{indoor_room_1_raw/triv_view_2.png}
    \end{tabular}} &
    \subfloat[UNet]{%
    \begin{tabular}{c}
         \expandafter\includegraphics\expandafter[\bullopts]{object_bull/unet_view_1.png} \\ 
         \expandafter\includegraphics\expandafter[\triopts]{object_triceratops_raw/unet_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfopts]{object_giraffe/unet_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfheadopts]{object_giraffe/unet_view_2.png} \\
         \expandafter\includegraphics\expandafter[\tikiopts]{object_tiki/unet_view_1.png} \\
         \expandafter\includegraphics\expandafter[\DSLRViewOneopts]{object_dslr/unet_view_1.png} \\
         \expandafter\includegraphics\expandafter[\roomZeroViewOneopts]{indoor_room_0_raw/unet_view_1.png} \\
         \expandafter\includegraphics\expandafter[\roomOneViewTwoopts]{indoor_room_1_raw/unet_view_2.png}
    \end{tabular}} &
    \subfloat[HPR]{%
    \begin{tabular}{c}
         \expandafter\includegraphics\expandafter[\bullopts]{object_bull/hpr_view_1.png} \\ 
         \expandafter\includegraphics\expandafter[\triopts]{object_triceratops_raw/hpr_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfopts]{object_giraffe/hpr_view_1.png} \\
         \expandafter\includegraphics\expandafter[\grfheadopts]{object_giraffe/hpr_view_2.png} \\
         \expandafter\includegraphics\expandafter[\tikiopts]{object_tiki/hpr_view_1.png} \\
         \expandafter\includegraphics\expandafter[\DSLRViewOneopts]{object_dslr/hpr_view_1.png} \\
         \expandafter\includegraphics\expandafter[\roomZeroViewOneopts]{indoor_room_0_raw/hpr_view_1.png} \\
         \expandafter\includegraphics\expandafter[\roomOneViewTwoopts]{indoor_room_1_raw/hpr_view_2.png}
    \end{tabular}} &
    \subfloat[Ours]{%
    \begin{tabular}{c}
        \expandafter\includegraphics\expandafter[\bullopts]{object_bull/ours_view_1.png} \\
        \expandafter\includegraphics\expandafter[\triopts]{object_triceratops_raw/ours_view_1.png} \\
        \expandafter\includegraphics\expandafter[\grfopts]{object_giraffe/ours_view_1.png} \\
        \expandafter\includegraphics\expandafter[\grfheadopts]{object_giraffe/ours_view_2.png} \\
        \expandafter\includegraphics\expandafter[\tikiopts]{object_tiki/ours_view_1.png} \\
        \expandafter\includegraphics\expandafter[\DSLRViewOneopts]{object_dslr/ours_angle_view_1.png} \\
        \expandafter\includegraphics\expandafter[\roomZeroViewOneopts]{indoor_room_0_raw/ours_view_1.png} \\
        \expandafter\includegraphics\expandafter[\roomOneViewTwoopts]{indoor_room_1_raw/ours_angle_view_2.png}
    \end{tabular}}
    \end{tabular}
    
    \caption{#1}
    \label{#2}
\end{figure}}
